Creation, Characterization, and Manipulation of Quantum Entanglement in a Photonic System

In this thesis, we report the theoretical and experimental investigations towards the creation, characterization, and manipulation of quantum entanglement in a photonic system. We examine two different aspects of quantum entanglement: In the first part, we discuss the experimental method for the preparation and characterization of SPDC-based polarization-entangled photon source. We provide a review study comparing different Entanglement Measures for non-maximally entangled two-qubit pure states and extend this analysis to higher-dimensional systems. In the second part, we study the entanglement dynamics of a two-qubit system in the presence of an Amplitude Damping Channel and present a scheme based on local unitary operations to protect entanglement from undergoing Entanglement Sudden Death. We extend the decoherence study to qubit-qutrit and qutrit-qutrit entangled systems and propose an entanglement protection scheme for the higher dimensional system.

==> append.tex <==
\appendix
\setcounter{chapter}{0}
\renewcommand{\chaptername}{Appendix}
%\renewcommand{\thechapter}{\arabic{section}.\arabic{ind}}
\renewcommand{\theequation}{\Alph{chapter}.\arabic{section}.\arabic{equation}}
\addcontentsline{toc}{chapter}{\numberline{}Appendix}
\setcounter{equation}{0}
\chapter{Basic and Auxiliary Results}
\section{Basic Results}

